Addressing Text Embedding Leakage in Diffusion-based Image Editing

Text-based image editing, powered by generative diffusion models, lets users modify images through natural-language prompts and has dramatically simplified traditional workflows. Despite these advances, current methods still suffer from a critical problem: attribute leakage, where edits meant for specific objects unintentionally affect unrelated regions or other target objects. Our analysis reveals the root cause as the semantic entanglement inherent in End-of-Sequence (EOS) embeddings generated by autoregressive text encoders, which indiscriminately aggregate attributes across prompts. To address this issue, we introduce Attribute-Leakage-free Editing (ALE), a framework that tackles attribute leakage at its source. ALE combines Object-Restricted Embeddings (ORE) to disentangle text embeddings, Region-Guided Blending for Cross-Attention Masking (RGB-CAM) for spatially precise attention, and Background Blending (BB) to preserve non-edited content. To quantitatively evaluate attribute leakage across various editing methods, we propose the Attribute-Leakage Evaluation Benchmark (ALE-Bench), featuring comprehensive editing scenarios and new metrics. Extensive experiments show that ALE reduces attribute leakage by large margins, thereby enabling accurate, multi-object, text-driven image editing while faithfully preserving non-target content.

==> ICCV2025/figures/cross_attention_example.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.12\linewidth}
        \centering
        \includegraphics[width=\linewidth]{ICCV2025/figures/images/paprika.pdf}
        \caption{Source image}
    \end{subfigure}
    \begin{subfigure}[b]{0.12\linewidth}
        \centering
        \includegraphics[width=\linewidth]{ICCV2025/figures/images/wrong_cross_attention.pdf}
        \caption{Edited image}
    \end{subfigure}
    \begin{subfigure}[b]{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{ICCV2025/figures/images/wrong_cross_attention_map.pdf}
        \caption{Visualization of cross-attention mappings}
        \label{fig:paprika cross-attention-leakage}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{
    {\color{blue} % attention map 그림 다시 뽑기
    Example of severe target-internal leakage in the cross-attention layer causing misplacement of target objects. 
    The task is to change ``\textit{yellow bell pepper}'' into ``\textbf{red apple}'' and ``\textit{red bell pepper}'' into `\textbf{`yellow cheese}''.
    However, due to unintended attention mappings, the positions of the target objects are swapped.
    Cross-attention mappings in Figure~\ref{fig:paprika cross-attention-leakage} are averaged across all timesteps.
    }
    }
    % \vspace{-0.5cm}
    \label{fig:paprika_cross_attention}
\end{figure*}

==> ICCV2025/sec/algorithms/EOS_embeddings.tex <==
\begin{algorithm}[t]
\caption{ORE}
\label{alg:object retricted embeddings}
\KwData{Object prompt list $[y_{1}, \dots, y_K]$ }
\KwResult{Object-restricted embedding set $E'=\{E'_{base}, E'_{1}, \dots, E'_K\}$}

\SetKwFunction{FEncoder}{$\text{Encoder}_{\text{text}}$}
\SetKwFunction{Flength}{$\text{len}$}
\SetKwFunction{Frange}{$\text{range}$}

$y_{base} \gets \text{`` and ''.join}([y_{1}, \dots, y_K])$; \\
$E'_{base} \gets \mathcal{E}_t(y_{base})$; \\
\For{$i \in \Frange(K)$}{
    $E'_{i} \gets \mathcal{E}_t(y_{i})$; \\
    $E'_{base}[y_i] \gets E'_{i}[y_i]$; \\
}
\Return $E'=\{E'_{base}, E'_{1}, \dots, E'_{K}\}$;
\end{algorithm}

==> ICCV2025/sec/algorithms/pipeline.tex <==
\begin{algorithm}[t!]
\caption{Attribute Leakage-free Edit}
\label{alg:pipeline}
\KwData{Source image $x^{S}$,
        prompt list $([y^{S}_{i}], [y^{T}_{i}])$,
        object mask list $m_{i}]$,
        Timestep schedule $[\tau_{N}, \tau_{N-1}, ... \tau_{0}]$
        }
\KwResult{Attribute-leakage-free Edited image $x^{T}$}

    \SetKwFunction{fEncoder}{$\text{Encoder}$}
    \SetKwFunction{fDecoder}{$\text{Decoder}$}
    \SetKwFunction{fORE}{$\text{ORE}$}
    \SetKwFunction{fSelfEdit}{$\text{Self-edit}$}
    \SetKwFunction{fRGBCAM}{$\text{RGB-CAM}$}
    \SetKwFunction{fBB}{$\text{BB}$}
    \SetKwFunction{fDDCM}{$\text{DDCM}$}
    \SetKwFunction{fInitLatent}{$\text{init\_latent}$}
    
    %$ $\\
    $z^{S} \gets \fEncoder(x^{S})$\;
    $E'[y^{S}_{i}], E'[y^{T}_{i}] \gets \fORE([y^{S}_{i}]), \fORE([y^{T}_{i}])$\;
    $z^{T}_{\tau_{N}} \sim \mathcal{N}(0, 1)$\;
    %$ $\\
    
    \For{$\tau_{i} \in [\tau_{N}, \tau_{N-1}, ... , \tau_{1}]$}{
        ${Q^{S}, K^{S}, V^{S}} \gets \epsilon_\theta(z^{S}_{\tau_{i}}, E'[y^{S}_{i}], \tau_{i})$\;
        ${Q^{T}, K^{T}, V^{T}} \gets \epsilon_\theta(z^{T}_{\tau_{i}}, E'[y^{T}_{i}], \tau_{i})$\;
        $Q, K, V \gets \fSelfEdit(\{Q^{S}, K^{S}, V^{S}\}, \{Q^{T}, K^{T}, V^{T}\}, \tau_{i})$\;
        ${A} \gets \fRGBCAM(Q, K, V, [m_{i}])$\;
        %$ $\\
        $z^{T}_{\tau_{i}} \gets \fDDCM(\epsilon_\theta, z^{T}_{\tau_{i}}, z^{S}, E'[y^{S}_{i}], E'[y^{T}_{i}], A)$\;
        $z^{T}_{\tau_{i-1}} \gets \fBB(z^{S}_{\tau_{i-1}}, z^{T}_{\tau_{i-1}}, m_{\text{back}})$\;
    }
    $x^{T} \gets \fDecoder(z^{T}_{\tau_{0}})$\;
    \Return $x^{T}$\;
\end{algorithm}


==> ICCV2025/sec/proposed_methods_algorithms.tex <==
%------------------------

\subsection{Object-Restricted Embeddings}
\label{sec:text_and_eos_embeddings}
A naive approach to eliminate the ambiguity of EOS embeddings is to fill it with zero vectors or to replace it with EOS embeddings of that from an empty prompt.
However, as shown in Figure~\ref{fig:EOS_modification}, such naive approaches generate images that do not match a text prompt, since a model is trained with EOS embeddings that have meaning.

To mitigate this issue, ORE modifies StructureDiffusion~\cite{feng2022training} to generate multiple lists of EOS embeddings, where each belongs to a single object.
In addition, the averaging process of cross-attention for multiple lists of EOS embeddings in StructureDiffusion is removed to block an interaction between independent embeddings.

For example, if $y_{1} = \text{``a red apple''}$ and $y_{2} = \text{``a yellow banana''}$, the base prompt becomes $y_{base} =\text{``a red apple and a yellow banana''}$ by concatenating all text prompts with the conjunction ``and''.
After constructing $y_i$, lists of token embeddings, $E = [e^{i}]$, are generated, where $E[y_i]$ represents embeddings made from $y_i$, that is, $E[y_{1} = \text{``a red apple''}]=[e_{\text{a}}^{1}, e_{\text{red}}^{2}, e_{\text{apple}}^{3}, e_{\text{EOS}}^{4}, e_{\text{EOS}}^{5}, ...]$.
Each $E[y_{i}]$ is made with an individual object prompt $y_i$ and independent of the other object prompts to restrict semantic influence within each object prompt.
As a result, when $n$ objects are specified, $(n+1)$ lists of embeddings are generated, including $y_{base}$.

\iffalse
%-------------------------------------------------------------------------
\subsection{Object-Restricted Embeddings}
\label{sec:text_and_eos_embeddings}
To address unintended semantic interactions among token embeddings in text-based image editing, we introduce \emph{ORE} in Algorithm~\ref{alg:object retricted embeddings}.
Unlike conventional methods, which typically encode a single global prompt embedding, we explicitly construct a separate, isolated embedding for each target object using ORE to minimize cross-token interference.

Text-to-image diffusion models typically use a single prompt embedding. 
In contrast, our editing problem provides prompts as pairs, necessitating the definition of distinct `base' prompts for the source and target.
We construct these base prompts by concatenating all text prompts in a given list, $[y_i]$, using the conjunction ``and'', applied to both the source and target object lists.
For example, if $y_{1} = \text{``a red apple''}$ and $y_{2} = \text{``a yellow banana''}$, the base prompt becomes $y_{base} =\text{``a red apple and a yellow banana''}$.
In this section, we use these $y_1$, $y_2$, and $y_{base}$ as default examples.

However, encoding $y_{base}$ directly with a text encoder $\mathcal{E}_t$ introduces undesirable semantic links between tokens.
For example, encoding $\mathcal{E}_t(y_{base})=[e_{\text{BOS}}^{0}, e_{\text{a}}^{1}, e_{\text{red}}^{2}, \dots, e_{\text{banana}}^{7}, e_{\text{EOS}}^{8}, \dots, e_{\text{EOS}}^{76}]$ may inadvertently allow  $e_{\text{red}}^{2}$ to influence $e_{\text{banana}}^{7}$, potentially resulting in undesired edits such as a red-colored banana~\cite{hu2024token} because of the auto-regressive nature of the CLIP text encoder.
Moreover, the EOS token embeddings $\{e_{\text{EOS}}^i\}$ frequently encapsulate global prompt information, intensifying cross-token interference through cross-attention mechanisms in diffusion models~\cite{hu2024token}.

To circumvent these pitfalls, ORE constructs distinct embeddings for individual object prompts $y_i$, effectively restricting semantic influence strictly within each object prompt.
In Algorithm~\ref{alg:object retricted embeddings}, we denote $E[y_i]$ as a list of token embeddings from $y_i$.
For example, $E[y_1]=[e_{\text{a}}^{1}, e_{\text{red}}^{2}, e_{\text{apple}}^{3}]$.
Because each ORE $E'_i$ is independently encoded using only the $y_i$, all token embeddings-including EOS embeddings-in $E'_i$ remain unaffected by other target attributes.
As a result, ORE enables generation of leakage-free prompt embeddings that we leverage in our subsequent method, region-guided blending for cross-attention layers.
\fi

\input{ICCV2025/sec/algorithms/EOS_embeddings}


% -------------------------------------------------------------------------
%     [  EOS Embeddings  ]    
% attribute leakage를 해결할 때, 의미를 가지는 단어들을 처리하는 것은 쉽다.
% 하지만 EOS는 그 자체로 의미를 가지지는 않고, EOS의 embedding이 의미를 가진다.
% 그러나 EOS의 embedding은 앞의 정보를 모두 포함하기 때문에, attribute leakage를 일으킬 수 있다.
% 이를 방지하기 위해 EOS를 0벡터로 만들거나 빈 문장에서 얻은 EOS의 embedding을 사용할 수 있다.
% 그러나 이는 출력물의 퀄리티가 상당히 떨어지는 결과로 이어지는데, 
% 이는 diffusion이 학습될 때 의미를 가지는 EOS로 학습했기 때문이다.
% (EOS 바꿨을 때 퀄리티 떨어지는 figure)
% EOS를 고려하지 않은 기존 method 중에 이를 bypass하는 method도 있다.
% RPG는 prompt를 rephrase하는 과정에서 서로 다른 object끼리 영향을 미치는 일이 없어진다.
% 하지만 그렇게 생성된 n개의 prompt는 각각 독립적으로 diffusion model을 거쳐야 하기 때문에,
% computational cost가 n배 늘어난다.
% 추가로, 이어붙인 부분에서 어색함이 없게 하기 위해 base prompt를 사용하는데,
% 이 또한 attribute leakage를 일으킬 여지가 있다.
% EOS의 문제와 computational leakage 문제를 해결하기 위해, 우리는 n개의 prompt를 만든다.
% 그러나 이로 인한 overhead가 크지 않도록, cross-attention에서만 n번의 계산을 한다.
% cross-attention에 관한 자세한 내용은 \ref{sec:cross-attention}
% (우리 알고리즘)
% -------------------------------------------------------------------------

% -------------------------------------------------------------------------
%     [  Cross-attention Masking  ]
% 
% -------------------------------------------------------------------------

\subsection{Region-Guided Blending for Cross-Attention Masking}
\label{sec:cross-attention masking}
A diffusion model takes a single list of text embeddings as input.
However, independent EOS embeddings for each object should be used to prevent attribute leakage.
We observed that, in U-Net architecture, which is commonly adopted in diffusion models, cross-attention layers are the only places where text embeddings are used. 
RGB-CAM modifies the mechanism of cross-attention to take as input lists of text embeddings, with a little overhead that is negligible in the overall diffusion process, as demonstrated in Table~\ref{table:time_complexity}.

First, we obtain a query $Q=W_q(z)$ from the target latent $z$ and a key $K=W_k(\mathcal{E}_t(y_{base}))$, producing a cross-attention map $M= \text{attention\_map}(Q,K)$.
$M$ is masked with $m_{i}$ per object and a region-specific cross-attention output $A_{i} = (M \odot m_i)*V_{i}$ is calculated, where $V_{i} = W_{v}(E[y_{i}])$ is a projection into a value.
The background region of the output is computed in the same way, using the background mask $m_{back}$ and $V_{base}$.
The final output of leakage-free cross-attention is computed as: $A=\Sigma_{i=1}^KA_i + (M \odot m_{back})*V_{base}$.
	
% Specifically, RGB-CAM uses segmentation masks $\{m_i\}$, generated by Grounded-SAM, to define spatial regions where $E[y_{i}]$ should exclusively attend.
% Then, a background mask $m_{back}$ is constructed by subtracting $\{m_i\}$ from a white image.

\iffalse
\subsection{Region-Guided Blending for Cross-Attention Masking}
\label{sec:cross-attention masking}
Naively applying ORE within the standard cross-attention layer can still lead to attribute leakage, because the standard cross-attention layer would restrict us to utilizing only a single ORE $E'_{base}$.
However, cross-attention maps corresponding to $E'_{base}[y_i]$ often attend to unintended regions, causing severe target-internal leakage in the generated images as illustrated in Figure~\ref{fig:paprika_cross_attention}.

To resolve this, \emph{RGB-CAM} (Algorithm~\ref{alg:rgb-cam}) explicitly restricts cross-attention outputs for OREs to their designated spatial regions in the target branch.
Specifically, RGB-CAM uses segmentation masks $\{m_i\}$, generated by Grounded-SAM, to define spatial regions where $y_i$ should exclusively attend.
Then, we construct a background mask $m_{back}$ by subtracting $\{m_i\}$ from a white image.

We then compute region-specific cross-attention outputs for each object and the background. First, we obtain a query $Q=W_q(z)$ from the target latent $z$ and a key $K=W_k(\mathcal{E}_t(y_{base}))$, yielding a cross-attention map $M= \text{attention\_map}(Q,K)$.
For each ORE $E'_i$, we project it into a value $V_i=W_v(E'_i)$.
Restricting $M$ with the corresponding mask $m_i$ multiplying it by $V_i$ yields a region-specific cross-attention output $A_i=(M \odot m_i)*V_i$.
The output background region is computed in the same way, using the background mask  $m_{back}$ and $V_{base}$.
The final leakage-free cross-attention output is then computed as: $A=\Sigma_{i=1}^KA_i + (M \odot m_{back})*V_{base}$.
By constraining attention to object-specific and background regions, RGB-CAM maintains spatial consistency and prevents attribute leakage, leading to high-quality image editing results.
\fi

\iffalse
\paragraph{Background blending}
\label{sec:background blending}
A previous approach to preserve backgrounds is local blending~\cite{hertz2022prompt}, which uses cross-attention maps to generate masks for background preservation. 
However, this method requires extensive trial and error to tune threshold values and becomes even more cumbersome when editing multiple objects.

To overcome these challenges, our \emph{Background Blending} method leverages the background mask $m_{back}$ to directly preserve non-target regions. 
At each denoising step $\tau$, BB blends the source branch latent $z^S_{\tau-1}$ for the background regions with the target branch latent $z^T_{\tau-1}$ for the edited regions, yielding a new target latent $\tilde{z}_{\tau-1}^T = m_{back} \odot z_{\tau-1}^S + (1 - m_{back}) \odot z_{\tau-1}^T$.
By relying on $z^S$ for non-target areas, BB preserves the original background and effectively reduces TE leakage.
\fi
\input{ICCV2025/sec/algorithms/Cross-attention_Masking}


\input{ICCV2025/figures/benchmark_examples}

\input{ICCV2025/figures/qualitative_comparison}
\input{ICCV2025/tables/metric_results}
\input{ICCV2025/tables/metric_results_per_object}
\input{ICCV2025/tables/metrics_results_per_edit_type}




%-------------------------------------------------------------------------
